Under Einstein's Microscope: Measuring Properties of Individual Rotating Massive Stars From Extragalactic Micro Caustic Crossings

Highly magnified stars residing in caustic crossing lensed galaxies at z ~ 0.7-1.5 in galaxy cluster lensing fields inevitably exhibit recurrent brightening events as they traverse a micro caustic network cast down by foreground intracluster stars. The detectable ones belong to Nature's most massive and luminous class of stars, with evolved blue supergiants being the brightest ones at optical wavelengths. Considering single stars in this work, we study to what extent intrinsic stellar parameters are measurable from multi-filter lightcurves, which can be obtained with optical/near-IR space telescopes during one or multiple caustic crossing events. We adopt a realistic model for the axisymmetric surface brightness profiles of rotating O/B stars and develop a numerical lensing code that treats finite-source-size effects. With a single micro caustic crossing, the ratio of the surface rotation velocity to the breakup value is measurable to an precision of ~ 0.1-0.2 for feasible observation parameters with current space telescopes, with all unknown intrinsic and extrinsic parameters marginalized over and without a degeneracy with inclination. Equatorial radius and bolometric luminosity can be measured to 1/3 and 2/3 of the fractional uncertainty in the micro caustic strength, for which the value is not known at each crossing but an informative prior can be obtained from theory. Parameter inference precision may be further improved if multiple caustic crossing events for the same lensed star are jointly analyzed. Our results imply new opportunities to survey individual massive stars in star-formation sites at z ~ 0.7-1.5 or beyond.

==> referee_report.tex <==
Reviewer:
This is a very interesting paper that explores the prospects of constraining the surface rotation (and other properties) of massive, gravitationally lensed stars at high redshifts. The basic idea is that the non-sphericity of a rapidly rotating star would introduce brightness and colour gradients across the surface of the star, which would result in chromatic effects in the measured light curve as the star crosses a microcaustic in a galaxy cluster lens. Given the many detections of lensed stars in recent years, and the many observational programs underway to detect lensed stars in galaxy cluster fields with both HST and JWST, I find this paper very timely. The ideas presented are novel and the paper is very well-written, and I would definitely recommend it for publication once the issues raised below have been addressed.

Major point:
1. My only real concern is about section 5 (mock parameter inference) and Figure 4. From the lower panel of Figure 4, it seems that the color variations when the star crosses the microcaustic are extremely small (~0.01-0.02 AB mag in F814W-F435W and F814W-F555W, based on the solid green and blue lines). Given that the assumed errors on the colors in each measurement are several times larger, I don't understand how the inference machinery can pick out the surface rotation parameter w in the way shown in Fig 5. How is it possible to distinguish the scattered mock data points from a case of no colour variation? Is the chromaticity only part of the information that the inference machinery is using, and most of the information is actually in the shape of the light curves (upper panel of Fig 4)? If so, this is not clearly spelled out in the paper, and should be added. Maybe it would be useful to show a model with a different rotation parameter w in the same light curve and color plots so that the reader can see the difference?

Minor points:
2. Part of my problem in grasping how the very impressive constraints of Figure 5 and 6 is possible from data of the type presented in Figure 4, may be that the authors don't really mention how much the brightness and colour of an unlensed star changes with viewing angle as one takes its non-sphericity (with the associated Teff and log(g) gradients) into account. They show the gradients in effective temperature (Figure 2), but don't really discuss how this translates into photometric properties. I think it would be useful if the authors could provide some representative numbers to guide the reader. For example: If one picks a star a certain location in the HR-diagram (Teff, log(L)) - how much can the integrated F555W AB magnitude and the integrated F435W-F814W colour change as one goes from w=0 to some higher value (for a couple of different viewing angles)?

3. It would be great if the authors could comment on whether non-axisymmetric features on the surfaces of massive stars could affect the measurements they propose. For instance, early-type B stars have been shown to display rotational variations with amplitudes of up to ~0.01 mag, which may be due to magnetically trapped, co-rotating features in the atmospheres of these stars (Balona, L.A. 2022, MNRAS 516, 3641).

4. Lines 65-66: "Several intriguing magnified star candidates have been reported in more distant lensed galaxies z ≃ 2-6 (Welch et al. 2022; Diego et al. 2023a,b; Furtak et al. 2024). If this is only meant to cover cases where z=2-6 stars are initially reported, the star covered by the Furtak et al. paper was actually first reported in Meena et al. 2023, ApJ 944, L6 (the Furtak et al. paper is about the follow-up spectroscopy). If it's meant to cover follow-up observations as well, then perhaps add Welch et al. 2022, ApJ 940, L1 (JWST observations of Earendel) to the list? The authors may also consider adding some reference to the lensed star candidate Godzilla, even though its nature is, perhaps, more controversial. For this, I would recommend Diego et al. 2022 A&A, 665, 134 (who argues that object Tr is a lensed star) or Vanzella et al. 2020, MNRAS, 499, L67 (who highlights Tr but does not clearly classify it as a lensed star).
